Lecture Notes on Stochastic Processes

This is lecture notes on the course "Stochastic Processes". In this format, the course was taught in the spring semesters 2017 and 2018 for third-year bachelor students of the Department of Control and Applied Mathematics, School of Applied Mathematics and Informatics at Moscow Institute of Physics and Technology. The base of this course was formed and taught for decades by professors from the Department of Mathematical Foundations of Control A.A. Natan, S.A. Guz, and O.G. Gorbachev. Besides standard chapters of stochastic processes theory (correlation theory, Markov processes) in this book (and lectures) the following chapters are included: von Neumann-Birkhoff-Khinchin ergodic theorem, macrosystem equilibrium concept, Markov Chain Monte Carlo, Markov decision processes and the secretary problem.

==> Section03/comments.tex <==
% стр. 76 где Действительно
%
% \begin{eqnarray*}
% \Exp ( Y - \hat{Y} )^{\top} A \left (Z - m_2 \right) = \Exp \left ( Y - m_1 -  R_{12}R_{22}^{-1} (Z - m_2) \right)^{\top} A \left (Z - m_2 \right)
% % &=& b + c\\
% % &=& d + e\\
% % && + d.
% \end{eqnarray*}

% $$\Exp ( Y - \hat{Y} )^{\top} A \left (Z - m_2 \right) = $$
% $$=\Exp \left ( Y - m_1 -  R_{12}R_{22}^{-1} (Z - m_2) \right)^{\top} A \left (Z - m_2 \right) =$$
% $$=\mathrm{tr\left(R_{12}A\right)} - \mathrm{tr\left(R_{12}R_{22}^{-1} R_{22}A\right)} = 0.$$

==> Section08/Comments.tex <==
\begin{comment}
\begin{theorem}[ (обратное уравнение Колмогорова)]
\textit{Пусть $X(t)$~-- марковский процесс с непрерывным временем и континуальным числом состояний. Кроме того, пусть выполняются следующие условия}:
\begin{enumerate}
    \item[1)] $\exists\, p_X(x,t\,|\,x_0,t_0) = \frac{d}{dx}F_X(x,t\,|\,x_0,t_0)$.
    \item[2)] $\exists \lim\limits_{\Delta t \to 0}\frac{1}{\Delta t}\int\limits_\R (y-x)^3 p_X(y,t+\Delta t\,|\,x,t)\,dy = 0$.
    \item[3)] ${\exists \lim\limits_{\Delta t \to 0}\frac{1}{\Delta t}\int\limits_\R (y-x)^2 p_X(y,t+\Delta t\,|\,x,t)\,dy = \sigma^2(t,x) \ge 0} \ \forall x, t.$ %{для всех $x, t$}, %$x$ и $t$;
    \item[4)] $\exists \lim\limits_{\Delta t \to 0}\frac{1}{\Delta t}\int\limits_\R (y-x) p_X(y,t+\Delta t\,|\,x,t)\,dy = a(t,x)\ \forall x, t.$% для всех $x$ и $t$.
\end{enumerate}
\textit{Тогда выполняется} \textit{обратное уравнение Колмогорова--Фоккера--План\-ка}:
% \begin{equation}
\begin{eqnarray}\label{eq:kolm_fok_pl_rev}
    -\frac{\partial p_X(x,t\,|\,x_0,t_0)}{\partial t_0} 
    &=& a(t_0, x_0) \frac{\partial p_X(x, t \,|\, x_0, t_0)}{\partial x_0} \notag+\\
    && + \ \frac{\sigma^2(t_0,x_0)}{2}\frac{\partial^2p_X(x,t\,|\,x_0,t_0)}{\partial x_0^2}.
\end{eqnarray}
% \end{equation}
\end{theorem}
\begin{proof}
    Разложим $p_X(x,t\,|\,x_1,t_1)$, как функцию от $x_1$ по формуле Тейлора с остаточным членом в форме Пеано в точке $x_0$ до членов третьего порядка малости включительно: 
    % \gav{Дальше идут формулы с очевидными overflow'ами; просьба их исправить!}\\
    % \egor{Форматирование нижних двух я изменил (до этого там использовалась техника, которую предложил Эдуард, но из-за этого происходил overfull).}
    \begin{multline*}
    p_X(x,t\,|\,x_1,t_1) = p_X(x,t\,|\,x_0,t_1) + \frac{\partial p_X(x,t\,|\,x_1,t_1)}{\partial x_1}\Bigg|_{x_1 = x_0}\cdot(x_1-x_0)+\\
        + \frac{1}{2!}\frac{\partial^2 p_X(x,t\,|\,x_1,t_1)}{\partial x_1^2}\Bigg|_{x_1 = x_0}\cdot(x_1-x_0)^2+\\
        + \frac{1}{3!}\frac{\partial^3 p_X(x,t\,|\,x_1,t_1)}{\partial x_1^3}\Bigg|_{x_1 = x_0}\cdot(x_1-x_0)^3 + o\left((x_1-x_0)^3\right).
    \end{multline*}
    % \begin{eqnarray*}
    %     p_X(x,t\,|\,x_1,t_1) &=& p_X(x,t\,|\,x_0,t_1) + \frac{\partial p_X(x,t\,|\,x_1,t_1)}{\partial x_1}\Bigg|_{x_1 = x_0}\cdot(x_1-x_0)\\
    %     &+& \frac{1}{2!}\frac{\partial^2 p_X(x,t\,|\,x_1,t_1)}{\partial x_1^2}\Bigg|_{x_1 = x_0}\cdot(x_1-x_0)^2\\
    %     &+& \frac{1}{3!}\frac{\partial^3 p_X(x,t\,|\,x_1,t_1)}{\partial x_1^3}\Bigg|_{x_1 = x_0}\cdot(x_1-x_0)^3 + o\left((x_1-x_0)^3\right).
    % \end{eqnarray*}
    Подставляя полученное разложение в формулу~\eqref{eq:cont_kolmogorov}, получим
    % \begin{eqnarray*}
    %     p_X(x,t\,|\,x_0,t_0) &=& p_X(x,t\,|\,x_0,t_1)\underbrace{\int\limits_{\R}p(x_1,t_1\,|\,x_0,t_0)dx_1}_{1}\\
    %     &+& \frac{\partial p_X(x,t\,|\,x_1,t_1)}{\partial x_1}\Bigg|_{x_1 = x_0}\int\limits_{\R}(x_1-x_0)p_X(x_1,t_1\,|\,x_0,t_0)dx_1\\
    %     &+& \frac{\partial^2 p_X(x,t\,|\,x_1,t_1)}{2\partial x_1^2}\Bigg|_{x_1 = x_0}\int\limits_{\R}(x_1-x_0)^2p_X(x_1,t_1\,|\,x_0,t_0)dx_1\\
    %     &+& o((t_1-t_0)),
    % \end{eqnarray*}
    
    \begin{multline*}
    p_X(x,t\,|\,x_0,t_0) = p_X(x,t\,|\,x_0,t_1)\underbrace{\int\limits_{\R}p(x_1,t_1\,|\,x_0,t_0)dx_1}_{1}+\\
        + \frac{\partial p_X(x,t\,|\,x_1,t_1)}{\partial x_1}\Bigg|_{x_1 = x_0}\int\limits_{\R}(x_1-x_0)p_X(x_1,t_1\,|\,x_0,t_0)dx_1+\\
        + \frac{\partial^2 p_X(x,t\,|\,x_1,t_1)}{2\partial x_1^2}\Bigg|_{x_1 = x_0}\int\limits_{\R}(x_1-x_0)^2p_X(x_1,t_1\,|\,x_0,t_0)dx_1+\\
        + o((t_1-t_0)),
    \end{multline*}
    где мы воспользовались свойством 2) из условия теоремы, чтобы записать члены, отвечающие за третий и более порядки малости, в виде $o(t_1-t_0)$. Осталось перенести $p_X(x,t\,|\,x_0,t_1)$ в левую часть, поделить обе части на $t_1-t_0$ и перейти к пределу при $t_1\to t_0$, чтобы получить уравнение \eqref{eq:kolm_fok_pl_rev}.
    \EndProof
\end{proof}
\end{comment}
%%\eduard{ЭГ: было бы здорово добавить сюда ссылку источник, где это уравнение есть в каком-то виде с доказательством.}

В условиях теоремы~8.1 справедливо также и \textit{прямое уравнение Колмогорова--Фоккера--Планка}, которое мы приводим без доказательства:
\begin{eqnarray*}
    \frac{\partial p_X(x,t\,|\,x_0,t_0)}{\partial t} &=& -\frac{\partial}{\partial x}\left(a(t_0,x_0) p_X(x,t\,|\,x_0,t_0)\right)+\\
    && + \ \frac{1}{2}\frac{\partial^2}{\partial x^2}\left(\sigma^2(t_0,x_0)p_X(x,t\,|\,x_0,t_0)\right).
\end{eqnarray*}
С доказательством можно ознакомиться в~\cite[глава 10, \S~54]{Gnedenko} (\textit{первое уравнение Колмогорова}).

\begin{example}
Винеровский процесс удовлетворяет всем условиям теоремы, причём ${a(t,x) = 0}$ и ${b(t,x) = 1}$. Если взять ${t_0 = 0, x_0 = X(t_0) = X(0) = 0$, то $p_X(x,t\,|\,x_0,t_0) = p_W(x,t)$ и из прямого уравнения Колмогорова--Фоккера--Планка следует, что
$$
    \frac{\partial p_W(x,t)}{\partial t} = \frac{1}{2}\frac{\partial^2p_W(x,t)}{\partial x^2}.\text{ \EndEx}
$$
\end{example}

==> Section09/backup.tex <==
\elena{КОММЕНТАРИЙ: Я так и не разобралась с решением ниже. не уверена, что студентам стоит в этом тоже разбираться. Я бы просто добавила предложение вида: Читатель, заинтересованный в получении точных формул для переходных вероятностей в дискретной и непрерывной модели Эренфестов, может посмотреть работы~\cite{Kac} и~\cite{Narita2001}. И также мне пока не удалось найти либо у себя, либо у Максима ошибку (так как ответы получились разные:(}

Перейдем теперь к вопросу о моменте времени, начиная с которого невязка между \gav{текущими} и предельными переходными вероятностями
\begin{equation}\label{eq:EhrenResidue}
    \Delta_{i,k}(t)=|p_{i,k}(t)-2^{-N}C_N^k|
\end{equation}
принимает значение не выше ${\varepsilon>0}$, т.е. ${\Delta_{i,k}(t)\le\varepsilon}$. Попробуем ответить на вопрос: как следует увеличить $t$ в зависимости от $N$ так, чтобы для нового значения $t$ невязка~\eqref{eq:EhrenResidue} оставалась в пределах $\varepsilon$?

Для этого воспользуемся явными выражениями для переходных вероятностей, их можно найти в работе~\cite{Narita2001}. В наших обозначениях

\begin{equation*}
p_{i,k}(t) = 2^{-N}C_N^k \sum\limits_{m=0}^N C_N^m K_i(m) K_k(m) \exp{(-2\lambda m t)},
\end{equation*}
где 
$$K_i(m)=(C_N^i)^{-1}\sum\limits_{l=0}^i (-1)^l C_m^l C_{N-m}^{i-l}, \ 0 < i \le N$$
и $K_0(m)=1$, $K_i(0)=1$. Заметим отсюда, что
$$p_{i,k}(t)-2^{-N}C_{N}^k=2^{-N}C_{N}^k\sum\limits_{m=1}^N C_{N}^m K_i(m) K_k(m) \exp{(-2\lambda m t)},$$ а значит:
$$\Delta_{i,k}(t) = \left|  \sum\limits_{m,l_1,l_2} f(N,i,k,l_1,l_2) \exp{(-2\lambda m t)} \right|,$$ где после сокращений $$f(N,i,k,m,l_1,l_2)=(-1)^{l_1+l_2} 2^{-N} C_N^m (C_N^i)^{-1}  C_m^{l_1} C_{N-m}^{i-l_1} C_m^{l_2} C_{N-m}^{i-l_2}, \ ik\ne0,$$
$$f(N,0,k,m,l_1,l_2)=(-1)^{l_2} 2^{-N} C_N^m C_m^{l_2} C_{N-m}^{i-l_2}, \ k\ne0,$$
$$f(N,i,0,m,l_1,l_2)=(-1)^{l_1} 2^{-N} C_N^m (C_N^i)^{-1}  C_m^{l_1} C_{N-m}^{i-l_1}, \ i\ne0,$$
$$f(N,0,0,m,l_1,l_2)=2^{-N} C_N^m.$$
Так как $\ln C_N^k=O(N\ln N)$, $N\to\infty$, то, как можно видеть, 
% \gav{Зачем здесь и далее модуль?} \eduard{Кажется, это по существу, функция $f$ может быть отрицательной.} 
$$\ag{\left|\ln |f(N,i,k,m,l_1,l_2)|\right|} = O(N \ln N), \ n\to\infty,$$ т.е. найдется постоянная $C$, такая, что для достаточно больших $N$ $$|\ln |f(N,i,k,m,l_1,l_2)|| \le C \cdot N \ln N.$$

Далее, $$\Delta_{i,k}(t) \le \sum\limits_{m,l_1,l_2} \left| f(N,i,k,l_1,l_2) \right| \exp{(-2\lambda t)},$$ откуда получаем, что при достаточно больших $N$

$$\Delta_{i,k}(t) \le N\cdot \max(ik,1)\cdot \exp{(C \cdot N \ln N)} \cdot \exp{(-2\lambda t)}.$$

Ограничивая правую часть этого выражения ${\varepsilon>0}$, приходим к неравенству 

$$\ln{N} + \ln{\max(ik,1)} + C\cdot N\ln{N} -2\lambda t \le \ln{\varepsilon}.$$

Это значит, что, начиная с некоторого $N$, найдется такая константа $D$, для которой \textit{достаточно} выбрать   произвольный момент времени ${t\ge D \cdot N \ln \ag{\left(N/\varepsilon\right)}}$, чтобы было выполнено неравенство ${\Delta_{i,k}(t) \le \varepsilon}$ для любых $i$ и $k$. 

% Другими словами, уже начиная с $t\sim N \ln N$, в хорошем приближении можно считать, что распределение вероятностей $p(t)$ независимо от стартового распределения совпадает со стационарным $\pi$.
